An Economic Solution to Copyright Challenges of Generative AI

Generative artificial intelligence (AI) systems are trained on large data corpora to generate new pieces of text, images, videos, and other media. There is growing concern that such systems may infringe on the copyright interests of training data contributors. To address the copyright challenges of generative AI, we propose a framework that compensates copyright owners proportionally to their contributions to the creation of AI-generated content. The metric for contributions is quantitatively determined by leveraging the probabilistic nature of modern generative AI models and using techniques from cooperative game theory in economics. This framework enables a platform where AI developers benefit from access to high-quality training data, thus improving model performance. Meanwhile, copyright owners receive fair compensation, driving the continued provision of relevant data for generative model training. Experiments demonstrate that our framework successfully identifies the most relevant data sources used in artwork generation, ensuring a fair and interpretable distribution of revenues among copyright owners.

==> corpus/pubmed_abstract.tex <==
The aim of the present work is to investigate the segmental movement patterns of the spine during normal treadmill gait. The spine movement during treadmill gait of ten healthy subjects (five men and five women) has been investigated using an optoelectronic measuring system. The spine was divided into seven segments, from C(7) to S(2). The subjects walked with their normal speed. All data were normalized to per cent of the gait cycle. The normal patterns of the spine segment movements were found in the sagittal and the frontal planes. The behaviour of the spine can be described as the motion of a stiff element with superimposed small, inter-segmental movements. These small inter-segmental movements were found both in the sagittal and the frontal planes. The small inter-segmental movements could play an important role in the reduction of the energy consumption during gait and in maintenance of the equilibrium. Any disability affecting the spine should result in changing spine movement pattern during gait, thus changing the overall gait pattern. Therefore, treatment and rehabilitation should not discard the influence of the spine malfunctioning, regardless of its nature.<|endoftext|>Nerve growth factor-stimulated mitogen-activated protein kinase activity is not necessary for neurite outgrowth of chick dorsal root ganglion sensory and sympathetic neurons.
Nerve growth factor (NGF)-stimulated neurite outgrowth in the rat PC12 tumor cell line recently has been shown to depend on the activation of the mitogen-activated protein (MAP) kinase kinase 1 (MEK1) (Pang et al.: J Biol Chem 270:13585-13588, 1995). In this study we have analyzed whether or not function of the MAP kinase pathway is necessary for NGF-stimulated neurite outgrowth in two subtypes of primary neurons derived from the embryonic chick peripheral nervous system (PNS). Treatment of p21ras-dependent dorsal root ganglion (DRG) sensory neurons (E9) with the MEK1 inhibitor PD98059 at concentrations up to 100 microM did not prevent NGF-stimulated neurite outgrowth. At this concentration NGF-stimulated tyrosine phosphorylation of MAP kinase p42 as well as MAP kinase activity both were decreased by approximately 80\%. Essentially the same results were obtained with p21ras-independent sympathetic neurons (E12). We conclude that, in contrast to the PC12 tumor cell line, NGF-stimulated MAP kinase activity is not necessary for neurite outgrowth of DRG sensory and sympathetic neurons derived from the chick PNS.<|endoftext|>Competitive promoter occupancy by two yeast paralogous transcription factors controlling the multidrug resistance phenomenon.
Highly flexible gene expression programs are required to allow cell growth in the presence of a wide variety of chemicals. We used genome-wide expression analyses coupled with chromatin immunoprecipitation experiments to study the regulatory relationships between two very similar yeast transcription factors involved in the control of the multidrug resistance phenomenon. Yrm1 (Yor172w) is a new zinc finger transcription factor, the overproduction of which decreases the level of transcription of the target genes of Yrr1, a zinc finger transcription factor controlling the expression of several membrane transporter-encoding genes. Surprisingly, the absence of YRR1 releases the transcriptional activity of Yrm1, which then up-regulates 23 genes, 14 of which are also direct target genes of Yrr1. Chromatin immunoprecipitation experiments confirmed that Yrm1 binds to the promoters of the up-regulated genes only in yeast strains from which YRR1 has been deleted. This sophisticated regulatory program can be associated with drug resistance phenotypes of the cell. The program-specific distribution of paired transcription factors throughout the genome may be a general mechanism by which similar transcription factors regulate overlapping gene expression programs in response to chemical stress.<|endoftext|>Sarcopenia predicts reduced survival in patients with hepatocellular carcinoma at first diagnosis.

==> math_command.tex <==
% \usepackage{cleveref}
\usepackage{bbm}

% \newtheorem{theorem}{Theorem}
% \newtheorem{lemma}[theorem]{Lemma}

% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{example}[theorem]{Example}
% \newtheorem{remark}{Remark}
% \newenvironment{claim}[1]{\par\noindent\underline{Claim:}\space#1}{}
% \newtheorem{remark-star}{Remark}
% \newtheorem{remark-star-1}{Remark}
% \newtheorem{conjecture}[theorem]{Conjecture}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{proposition}[theorem]{Proposition}
\usepackage{booktabs}
\newcommand{\fix}{\marginpar{FIX}}
\newcommand{\new}{\marginpar{NEW}}


\newtheorem{innercustomthm}{Theorem}
\newenvironment{customthm}[1]
  {\renewcommand\theinnercustomthm{#1}\innercustomthm}
  {\endinnercustomthm}



\newcommand{\E}{\mathbb{E}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\eps}{\varepsilon}
\newcommand{\D}{\mathcal{D}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\N}{\mathcal{N}}
\newcommand{\I}{\mathcal{I}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\Ind}{\mathds{1}}
\newcommand{\g}{\nabla}
\newcommand{\iden}{\bm{1}}
\newcommand{\inner}[2]{\left\langle #1, #2 \right\rangle}

\newcommand{\ind}{\mathbbm{1}}

\newcommand{\A}{\mathcal{A}}

\newcommand{\U}{v}
\newcommand{\test}{\mathrm{val}}
\newcommand{\Utot}{U_{\mathrm{tot}}}
\newcommand{\metric}{\texttt{acc}}

\newcommand{\unif}{\mathrm{Unif}}
\newcommand{\semi}{\mathrm{semi}}
\newcommand{\shap}{\mathrm{shap}}
\newcommand{\loo}{\mathrm{loo}}
\newcommand{\banz}{\mathrm{banz}}

\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}
% \newcommand{\MS}{\texttt{MultiSet}}

\newcommand{\MS}{ \mathbb{N}^\cX }

\newcommand{\NBK}{ \texttt{NB}_{x^{(\test)}, K} }


\newcommand{\NBtauxval}{ \texttt{NB}_{x^{(\test)}, \tau} }

\newcommand{\NBxtau}{ \texttt{NB}_{x, \tau} }

\newcommand{\NBxtaun}{ \texttt{NB}_{x, \tau_n} }

\newcommand{\cn}{ \mathbf{c} }
\newcommand{\ctau}{\mathbf{c}_{x^{(\test)}, \tau}}
\newcommand{\cA}{\mathbf{c}_{z^{(\test)}, \tau}^{ (+) }}

\newcommand{\DPcn}{ \widehat{\mathbf{c}} }
\newcommand{\DPctau}{\widehat{\mathbf{c}}_{x^{(\test)}, \tau}}
\newcommand{\DPcA}{\widehat{\mathbf{c}}_{z^{(\test)}, \tau}^{ (+) }}

\newcommand{\round}{ \texttt{round} }

\newcommand{\subsample}{ \texttt{sample} }

\newcommand{\supp}{ \texttt{supp} }

\newcommand{\knn}{ \texttt{KNN} }

\newcommand{\knnold}{ \texttt{KNN-OLD} }

\newcommand{\tknn}{ \texttt{TKNN} }

\newcommand{\Dval}{ D^{(\test)} }

\newcommand{\Nval}{ N^{(\test)} }

\newcommand{\Ct}{\textbf{C}_{ z^{(\test)} }}
\newcommand{\DPCt}{ \widehat{\textbf{C}}_{ z^{(\test)} } }

\newcommand{\red}[1]{\textcolor[RGB]{255, 49, 49}{#1}}
\newcommand{\green}[1]{\textcolor[RGB]{34,169,34}{#1}}
\newcommand{\blue}[1]{\textcolor[RGB]{0,0,245}{#1}}

\newcommand{\cmt}[1]{\texttt{// #1}}

\newcommand{\shapvalue}{\text{KNNSV}}
\newcommand{\Datk}{D_{\text{shadow}}}
\newcommand{\phiobs}{\phi_{\text{obs}}}

\newcommand{\mS}{\mathbf{S}}

\newcommand{\zval}{ z^{(\test)} }
\newcommand{\xval}{ x^{(\test)} }
\newcommand{\yval}{ y^{(\test)} }

\newcommand{\xgen}{x^{(\text{gen})}}
\newcommand{\Xgen}{X^{(\text{gen})}}

\newcommand{\C}{\mathbf{C}}
\newcommand{\Dsort}{\widetilde{D}}
\newcommand{\weightfunc}{\omega_{\xval}}

\usepackage{tikz}

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=1pt] (char) {#1};}}

\newcommand{\Gi}{\texttt{G}_i}
\newcommand{\Gil}{\texttt{G}_{i, \ell}}
\newcommand{\Gizero}{\texttt{G}_{i, 0}}

\newcommand{\Gitil}{\widetilde{\texttt{G}}_i}
\newcommand{\Giltil}{\Gitil(\ell)}

\newcommand{\Fi}{\texttt{F}_i}
\newcommand{\Fihat}{\widehat{\texttt{F}}_i}

\newcommand{\Ri}{\texttt{R}_i}
\newcommand{\Rim}{\texttt{R}_{i, m}}
\newcommand{\Ritil}{\widetilde{\texttt{R}}_i}

\newcommand{\Rimhat}{\widehat{\texttt{R}}_{i, m}}

\newcommand{\wspace}{\texttt{V}}
\newcommand{\nwspace}{V}

\newcommand{\s}{\mathbf{s}}
\newcommand{\e}{\mathbf{e}}

\newcommand{\mstar}{M^\star}
\newcommand{\phihat}{\widehat \phi}
\newcommand{\phihatmstar}{\phihat_{z_i}^{(\mstar)}}

\newcommand{\sign}{ \texttt{sign} }

\newcommand{\logo}{FlickrLogo-27}

\renewcommand{\cmt}[1]{\texttt{// #1}}

\newcommand{\wtil}{\widetilde{w}}

\newcommand{\SRS}{\texttt{SRS}}

\newcommand{\Di}{D^{(i)}}
\newcommand{\Dj}{D^{(j)}}

\newcommand{\playerset}{\mathcal{P}}
\newcommand{\mE}{\mathcal{E}}
\newcommand{\mG}{\mathcal{G}}
\newcommand{\aicomp}{\texttt{AI-Dev}}
\newcommand{\ShareData}{ \beta_{\text{data}} }


\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}


\newif\ifinappendix




